Learning from few examples: Classifying sex from retinal images via deep learning

Deep learning has seen tremendous interest in medical imaging, particularly in the use of convolutional neural networks (CNNs) for developing automated diagnostic tools. The facility of its non-invasive acquisition makes retinal fundus imaging amenable to such automated approaches. Recent work in analyzing fundus images using CNNs relies on access to massive data for training and validation - hundreds of thousands of images. However, data residency and data privacy restrictions stymie the applicability of this approach in medical settings where patient confidentiality is a mandate. Here, we showcase results for the performance of DL on small datasets to classify patient sex from fundus images - a trait thought not to be present or quantifiable in fundus images until recently. We fine-tune a Resnet-152 model whose last layer has been modified for binary classification. In several experiments, we assess performance in the small dataset context using one private (DOVS) and one public (ODIR) data source. Our models, developed using approximately 2500 fundus images, achieved test AUC scores of up to 0.72 (95% CI: [0.67, 0.77]). This corresponds to a mere 25% decrease in performance despite a nearly 1000-fold decrease in the dataset size compared to prior work in the literature. Even with a hard task like sex categorization from retinal images, we find that classification is possible with very small datasets. Additionally, we perform domain adaptation experiments between DOVS and ODIR; explore the effect of data curation on training and generalizability; and investigate model ensembling to maximize CNN classifier performance in the context of small development datasets.

==> author_summary.tex <==
% Please keep the Author Summary between 150 and 200 words
% Use first person. PLOS ONE authors please skip this step. 
% Author Summary not valid for PLOS ONE submissions.   
\section*{Author summary}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% reftex-default-bibliography: ("/Users/aberk/Dropbox/org/bibliography.bib")
%%% End:


==> background.tex <==

\section{Background}
\label{sec:background}

\edit{We will not be using a background section. This information will be split:
  high-level pieces going into Methods, with the content supporting them
  relocated to the appendix or supplemenatry materials.}








%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% reftex-default-bibliography: ("/Users/aberk/Dropbox/org/bibliography.bib")
%%% End:


==> naive_ensembling.tex <==





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% reftex-default-bibliography: ("/Users/aberk/Dropbox/org/bibliography.bib")
%%% End:


==> related_work.tex <==
\section{Related Work}
\label{sec:related-work}



\edit{We will not be using a related work section; see the Introduction for what
  would normally go here.}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% End:


==> reshuffled_ensembling.tex <==
\subsection{Reshuffled ensembling}
\label{sec:results-reshuf-ensembling}


Denote a collection of data $\mathcal{D} = \mathcal{S} \cup \mathcal{T}$, the
union of a development and test set, where
$\mathcal{S} := \{ (x_{i}, y_{i}) : i \in [m_{\mathcal{S}}]\}$ and
$\mathcal{T} := \{ (x_{i}, y_{i}) : i \in [m_{\mathcal{T}}]\}$. Denote by
$\mathcal{A}$ the training algorithm. For an ensemble of $n$ models, we
generate $\{f_{j}\}_{j=1}^{n}$ in the following way. Partition
$\mathcal{S} := \mathcal{U}_{j}\cup \mathcal{V}_{j}$, where $\mathcal{U}_{j}$
is the training set and $\mathcal{V}_{j}$ is a validation set. Run the
algorithm $\mathcal{A}(\mathcal{U}_{j}; \mathcal{V}_{j})$ using the training
data until $f_{j}$ achieves good performance on the test set. Define the model
$F_{\mathrm{ens}}(\cdot) := \frac{1}{n} \sum_{j=1}^{n} f_{j}(\cdot)$. By
construction, $\mathrm{range}(f_{j}) \in [0, 1]$, and so $F_{\mathrm{ens}}$ has
this property, too. 


\begin{figure}[h]
  \centering
  \includegraphics[width=.45\textwidth]{fig/ensemble/test-roc-auc_by_num-ensembled.pdf}
 \qquad  \includegraphics[width=.45\textwidth]{fig/ensemble/mean-val-roc-auc-by-ensemble-test-roc-auc.pdf}
 \caption{\textbf{Left:} A plot of the ROC AUC score on the test dataset for an
   ensemble, as a function of the number of models in that ensemble. The orange
   line depicts the mean test ROC AUC score, where the mean is taken over all
   ensembles of a certain size. The orange bars about the mean represent
   approximate $95\%$ confidence intervals for the ROC AUC score on the test
   set. \textbf{Right:} A scatter plot visualizing the correspondence between
   the mean ROC AUC score on the validation set of each model used in an
   ensemble, and the ROC AUC score on the test set of the ensemble of those
   models. A simple linear regression on the data found a relationship
   $\mathrm{AUC}_{\mathrm{test}} = 0.5538\mathrm{meanAUC}_{\mathrm{val}} +
   0.2784$ (adjusted $R^{2} = 0.319$).}
  \label{fig:shuf1}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=.45\textwidth]{fig/ensemble/val-roc-auc_by_num-ensembled.pdf}
  \qquad
  \includegraphics[width=.45\textwidth]{fig/ensemble/val-roc-auc_by_test-roc-auc.pdf}
  \caption{\textbf{Left:} A plot of the validation ROC AUC for an ensemble as a
    function of the number of models in that ensemble. The orange line depicts
    the mean validation ROC AUC, and the orange bars about it represent
    approximate $95\%$ confidence intervals. \textbf{Right:} A scatter plot
    depicting the correspondence between the ensemble's validation ROC AUC
    score and its test ROC AUC score. A simple linear regression on the data
    yields a correlation coefficient of $\rho = 0.109$ ($R^{2} = 0.150$). }
  \label{fig:shuf2}
\end{figure}


\begin{center}
  \begin{tabular}{llllllrrr}
    \toprule
    {} & $\mathrm{AUC}_{\mathrm{val}}$ & $\mathrm{ACC}_{\mathrm{val}}$ &
    $\mathrm{minAUC}_{\mathrm{val}}$ & $\mathrm{maxAUC}_{\mathrm{val}}$ & %
    $\mathrm{meanAUC}_{\mathrm{val}}$ & intercept & $R^{2}$ & $\mathrm{MAE}$ \\
    \midrule
    0 & 0.109 & $\times$ & $\times$ & $\times$ & $\times$ & 0.563 & 0.150 & 0.008 \\
    1 & $\times$ & 0.104 & $\times$ & $\times$ & $\times$ & 0.576 & 0.109 & 0.008 \\
    2 & $\times$ & $\times$ & 0.134 & $\times$ & $\times$ & 0.567 & 0.107 & 0.008 \\
    3 & $\times$ & $\times$ & $\times$ & 0.427 & $\times$ & 0.350 & 0.243 & 0.008 \\
    4 & $\times$ & $\times$ & $\times$ & $\times$ & 0.554 & 0.278 & 0.320 & 0.007 \\
    5 & $\times$ & $\times$ & 0.132 & 0.423 & $\times$ & 0.269 & 0.346 & 0.007 \\
    6 & $\times$ & $\times$ & 0.030 & 0.254 & 0.335 & 0.227 & 0.362 & 0.007 \\
    7 & 0.052 & 0.029 & 0.158 & 0.283 & $\times$ & 0.288 & 0.389 & 0.007 \\
\bottomrule
\end{tabular}

\end{center}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% reftex-default-bibliography: ("/Users/aberk/Dropbox/org/bibliography.bib")
%%% End:


==> results_ensemble.tex <==
% \section{Results: Ensembling}
% \label{sec:results-ensembling}

% \input{naive_ensembling}

% \input{reshuffled_ensembling}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dlri.tex"
%%% reftex-default-bibliography: ("/Users/aberk/Dropbox/org/bibliography.bib")
%%% End:

